Distributionally-Informed Recommender System Evaluation

Current practice for evaluating recommender systems typically focuses on point estimates of user-oriented effectiveness metrics or business metrics, sometimes combined with additional metrics for considerations such as diversity and novelty. In this paper, we argue for the need for researchers and practitioners to attend more closely to various distributions that arise from a recommender system (or other information access system) and the sources of uncertainty that lead to these distributions. One immediate implication of our argument is that both researchers and practitioners must report and examine more thoroughly the distribution of utility between and within different stakeholder groups. However, distributions of various forms arise in many more aspects of the recommender systems experimental process, and distributional thinking has substantial ramifications for how we design, evaluate, and present recommender systems evaluation and research results. Leveraging and emphasizing distributions in the evaluation of recommender systems is a necessary step to ensure that the systems provide appropriate and equitably-distributed benefit to the people they affect.

==> case-study/ItemDists/item-dist-tbl.tex <==
\begin{tabular}{lrrr}
\toprule
{} &      Gini &        L2 &        KL \\
\midrule
IALS &  0.732345 &  0.000329 &  0.424431 \\
IKNN &  0.988025 &  0.025326 &  1.993307 \\
Pop  &  0.995073 &  0.051245 &  2.398029 \\
\bottomrule
\end{tabular}


==> case-study/UserDists/metric-point-estimates.tex <==
\begin{tabular}{lrrrrrrr}
 & RBP & rbp05 & HR & HR@10 & HR@20 & nDCG & MRR \\
algo &  &  &  &  &  &  &  \\
IALS & \font-weightbold 0.061390 & 0.045218 & \font-weightbold 1.000000 & \font-weightbold 0.494667 & \font-weightbold 0.680667 & \font-weightbold 0.286168 & 0.223139 \\
IKNN & 0.057128 & \font-weightbold 0.051729 & \font-weightbold 1.000000 & 0.448000 & 0.594000 & 0.261441 & \font-weightbold 0.237165 \\
Pop & 0.035225 & 0.030296 & 0.996000 & 0.302000 & 0.452000 & 0.210809 & 0.154980 \\
\end{tabular}


==> cf-example.tex <==
\resizebox{\columnwidth}{!}{
\begin{tabular}{lccccc}
Algorithm
& Mean
& 10\%ile
& Median
& 90\%ile
& Dist. (KDE) \\
\toprule
Implicit MF &
\begin{tabular}{@{}c@{}}%
0.211 \\%
{\smaller[2] (0.210, 0.212)}\end{tabular} &
\begin{tabular}{@{}c@{}}%
0.029 \\%
{\smaller[2] (0.027, 0.031)}\end{tabular} &
\begin{tabular}{@{}c@{}}%
0.165 \\%
{\smaller[2] (0.164, 0.166)}\end{tabular} &
\begin{tabular}{@{}c@{}}%
0.466 \\%
{\smaller[2] (0.463, 0.469)}\end{tabular} &
\begin{sparkline}{9}
\sparkdot 0.211 0.284 red
\spark
  0.000 0.319
  0.020 0.266
  0.041 0.344
  0.061 0.407
  0.082 0.391
  0.102 0.422
  0.122 0.405
  0.143 0.381
  0.163 0.356
  0.184 0.324
  0.204 0.294
  0.224 0.264
  0.245 0.238
  0.265 0.215
  0.286 0.195
  0.306 0.174
  0.327 0.153
  0.347 0.135
  0.367 0.121
  0.388 0.110
  0.408 0.098
  0.429 0.089
  0.449 0.082
  0.469 0.076
  0.490 0.070
  0.510 0.063
  0.531 0.057
  0.551 0.052
  0.571 0.047
  0.592 0.043
  0.612 0.039
  0.633 0.035
  0.653 0.030
  0.673 0.026
  0.694 0.023
  0.714 0.020
  0.735 0.017
  0.755 0.016
  0.776 0.014
  0.796 0.012
  0.816 0.011
  0.837 0.009
  0.857 0.008
  0.878 0.007
  0.898 0.006
  0.918 0.005
  0.939 0.004
  0.959 0.002
  0.980 0.001
  1.000 0.001
  /
\end{sparkline}
\\
Implicit II &
\begin{tabular}{@{}c@{}}%
0.221 \\%
{\smaller[2] (0.220, 0.222)}\end{tabular} &
\begin{tabular}{@{}c@{}}%
0.000 \\%
{\smaller[2] (0.000, 0.000)}\end{tabular} &
\begin{tabular}{@{}c@{}}%
0.154 \\%
{\smaller[2] (0.153, 0.155)}\end{tabular} &
\begin{tabular}{@{}c@{}}%
0.528 \\%
{\smaller[2] (0.525, 0.531)}\end{tabular} &
\begin{sparkline}{9}
\sparkdot 0.221 0.177 red
\spark
  0.000 0.434
  0.020 0.378
  0.041 0.381
  0.061 0.427
  0.082 0.389
  0.102 0.365
  0.122 0.338
  0.143 0.300
  0.163 0.262
  0.184 0.227
  0.204 0.197
  0.224 0.174
  0.245 0.158
  0.265 0.148
  0.286 0.144
  0.306 0.144
  0.327 0.143
  0.347 0.144
  0.367 0.143
  0.388 0.138
  0.408 0.129
  0.429 0.119
  0.449 0.109
  0.469 0.099
  0.490 0.089
  0.510 0.081
  0.531 0.074
  0.551 0.067
  0.571 0.062
  0.592 0.057
  0.612 0.052
  0.633 0.048
  0.653 0.044
  0.673 0.041
  0.694 0.037
  0.714 0.033
  0.735 0.028
  0.755 0.025
  0.776 0.023
  0.796 0.020
  0.816 0.017
  0.837 0.015
  0.857 0.013
  0.878 0.011
  0.898 0.009
  0.918 0.007
  0.939 0.005
  0.959 0.003
  0.980 0.002
  1.000 0.001
  /
\end{sparkline}
\\
Popular &
\begin{tabular}{@{}c@{}}%
0.135 \\%
{\smaller[2] (0.134, 0.136)}\end{tabular} &
\begin{tabular}{@{}c@{}}%
0.000 \\%
{\smaller[2] (0.000, 0.000)}\end{tabular} &
\begin{tabular}{@{}c@{}}%
0.087 \\%
{\smaller[2] (0.086, 0.088)}\end{tabular} &
\begin{tabular}{@{}c@{}}%
0.360 \\%
{\smaller[2] (0.357, 0.362)}\end{tabular} &
\begin{sparkline}{9}
\sparkdot 0.135 0.318 red
\spark
  0.000 0.999
  0.020 0.500
  0.041 0.516
  0.061 0.596
  0.082 0.454
  0.102 0.418
  0.122 0.359
  0.143 0.298
  0.163 0.253
  0.184 0.214
  0.204 0.182
  0.224 0.155
  0.245 0.134
  0.265 0.121
  0.286 0.110
  0.306 0.104
  0.327 0.096
  0.347 0.089
  0.367 0.082
  0.388 0.077
  0.408 0.070
  0.429 0.062
  0.449 0.055
  0.469 0.049
  0.490 0.046
  0.510 0.041
  0.531 0.036
  0.551 0.030
  0.571 0.024
  0.592 0.019
  0.612 0.015
  0.633 0.012
  0.653 0.011
  0.673 0.009
  0.694 0.007
  0.714 0.006
  0.735 0.005
  0.755 0.005
  0.776 0.004
  0.796 0.003
  0.816 0.003
  0.837 0.002
  0.857 0.001
  0.878 0.001
  0.898 0.000
  0.918 0.000
  0.939 0.000
  0.959 0.000
  0.980 0.000
  1.000 0.000
  /
\end{sparkline}
\\
\bottomrule
\end{tabular}
}

==> deep-example.tex <==
\begin{tabular}{lccccc}
System
& Mean
& 10\%ile
& Median
& 90\%ile
& Dist. (KDE) \\
\toprule
1 &
0.965 &
1.000 &
1.000 &
1.000 &
\begin{sparkline}{9}
\sparkdot 0.965 0.911 red
\spark
  0.000 0.028
  0.020 0.031
  0.041 0.032
  0.061 0.032
  0.082 0.030
  0.102 0.028
  0.122 0.025
  0.143 0.021
  0.163 0.017
  0.184 0.013
  0.204 0.009
  0.224 0.006
  0.245 0.004
  0.265 0.003
  0.286 0.001
  0.306 0.001
  0.327 0.000
  0.347 0.000
  0.367 0.000
  0.388 0.000
  0.408 0.000
  0.429 0.000
  0.449 0.000
  0.469 0.000
  0.490 0.000
  0.510 0.000
  0.531 0.000
  0.551 0.000
  0.571 0.000
  0.592 0.000
  0.612 0.000
  0.633 0.000
  0.653 0.000
  0.673 0.000
  0.694 0.001
  0.714 0.002
  0.735 0.005
  0.755 0.011
  0.776 0.023
  0.796 0.044
  0.816 0.080
  0.837 0.136
  0.857 0.217
  0.878 0.325
  0.898 0.458
  0.918 0.607
  0.939 0.755
  0.959 0.883
  0.980 0.969
  1.000 1.000
  /
\end{sparkline}
\\
bert\_6 &
0.900 &
0.500 &
1.000 &
1.000 &
\begin{sparkline}{9}
\sparkdot 0.900 0.431 red
\spark
  0.000 0.024
  0.020 0.027
  0.041 0.030
  0.061 0.033
  0.082 0.035
  0.102 0.038
  0.122 0.040
  0.143 0.041
  0.163 0.043
  0.184 0.043
  0.204 0.043
  0.224 0.043
  0.245 0.042
  0.265 0.041
  0.286 0.040
  0.306 0.039
  0.327 0.040
  0.347 0.041
  0.367 0.043
  0.388 0.046
  0.408 0.049
  0.429 0.052
  0.449 0.055
  0.469 0.056
  0.490 0.057
  0.510 0.056
  0.531 0.054
  0.551 0.051
  0.571 0.046
  0.592 0.041
  0.612 0.036
  0.633 0.032
  0.653 0.029
  0.673 0.028
  0.694 0.030
  0.714 0.037
  0.735 0.049
  0.755 0.068
  0.776 0.094
  0.796 0.130
  0.816 0.174
  0.837 0.228
  0.857 0.289
  0.878 0.356
  0.898 0.425
  0.918 0.491
  0.939 0.549
  0.959 0.594
  0.980 0.624
  1.000 0.634
  /
\end{sparkline}
\\
bigIR{-}T5xp{-}T5{-}F &
0.925 &
0.650 &
1.000 &
1.000 &
\begin{sparkline}{9}
\sparkdot 0.925 0.569 red
\spark
  0.000 0.025
  0.020 0.027
  0.041 0.029
  0.061 0.030
  0.082 0.030
  0.102 0.029
  0.122 0.027
  0.143 0.025
  0.163 0.023
  0.184 0.021
  0.204 0.020
  0.224 0.019
  0.245 0.020
  0.265 0.021
  0.286 0.022
  0.306 0.025
  0.327 0.028
  0.347 0.031
  0.367 0.035
  0.388 0.039
  0.408 0.043
  0.429 0.046
  0.449 0.049
  0.469 0.051
  0.490 0.051
  0.510 0.050
  0.531 0.047
  0.551 0.043
  0.571 0.037
  0.592 0.032
  0.612 0.026
  0.633 0.021
  0.653 0.017
  0.673 0.014
  0.694 0.015
  0.714 0.018
  0.735 0.026
  0.755 0.041
  0.776 0.063
  0.796 0.096
  0.816 0.142
  0.837 0.201
  0.857 0.273
  0.878 0.357
  0.898 0.448
  0.918 0.539
  0.939 0.623
  0.959 0.690
  0.980 0.734
  1.000 0.750
  /
\end{sparkline}
\\
bl\_bcai\_mdl1\_vs &
0.858 &
0.333 &
1.000 &
1.000 &
\begin{sparkline}{9}
\sparkdot 0.858 0.288 red
\spark
  0.000 0.037
  0.020 0.041
  0.041 0.045
  0.061 0.048
  0.082 0.051
  0.102 0.054
  0.122 0.056
  0.143 0.058
  0.163 0.060
  0.184 0.061
  0.204 0.063
  0.224 0.064
  0.245 0.064
  0.265 0.065
  0.286 0.066
  0.306 0.067
  0.327 0.067
  0.347 0.068
  0.367 0.068
  0.388 0.069
  0.408 0.068
  0.429 0.068
  0.449 0.067
  0.469 0.065
  0.490 0.063
  0.510 0.060
  0.531 0.057
  0.551 0.053
  0.571 0.049
  0.592 0.046
  0.612 0.043
  0.633 0.042
  0.653 0.043
  0.673 0.046
  0.694 0.053
  0.714 0.064
  0.735 0.079
  0.755 0.101
  0.776 0.127
  0.796 0.160
  0.816 0.198
  0.837 0.241
  0.857 0.286
  0.878 0.333
  0.898 0.379
  0.918 0.421
  0.939 0.457
  0.959 0.485
  0.980 0.503
  1.000 0.508
  /
\end{sparkline}
\\
DLH\_d\_5\_t\_25 &
0.717 &
0.100 &
1.000 &
1.000 &
\begin{sparkline}{9}
\sparkdot 0.717 0.103 red
\spark
  0.000 0.089
  0.020 0.095
  0.041 0.101
  0.061 0.106
  0.082 0.110
  0.102 0.114
  0.122 0.116
  0.143 0.119
  0.163 0.120
  0.184 0.121
  0.204 0.121
  0.224 0.120
  0.245 0.119
  0.265 0.117
  0.286 0.115
  0.306 0.113
  0.327 0.110
  0.347 0.107
  0.367 0.104
  0.388 0.100
  0.408 0.096
  0.429 0.092
  0.449 0.088
  0.469 0.084
  0.490 0.080
  0.510 0.077
  0.531 0.073
  0.551 0.071
  0.571 0.069
  0.592 0.069
  0.612 0.070
  0.633 0.072
  0.653 0.076
  0.673 0.083
  0.694 0.091
  0.714 0.101
  0.735 0.114
  0.755 0.129
  0.776 0.146
  0.796 0.164
  0.816 0.184
  0.837 0.204
  0.857 0.224
  0.878 0.243
  0.898 0.261
  0.918 0.277
  0.939 0.289
  0.959 0.299
  0.980 0.305
  1.000 0.307
  /
\end{sparkline}
\\
DoRA\_Large &
0.157 &
0.000 &
0.000 &
0.850 &
\begin{sparkline}{9}
\sparkdot 0.157 0.303 red
\spark
  0.000 0.457
  0.020 0.459
  0.041 0.453
  0.061 0.439
  0.082 0.418
  0.102 0.392
  0.122 0.361
  0.143 0.327
  0.163 0.292
  0.184 0.257
  0.204 0.224
  0.224 0.192
  0.245 0.164
  0.265 0.138
  0.286 0.117
  0.306 0.098
  0.327 0.083
  0.347 0.071
  0.367 0.062
  0.388 0.055
  0.408 0.050
  0.429 0.046
  0.449 0.043
  0.469 0.041
  0.490 0.039
  0.510 0.037
  0.531 0.035
  0.551 0.033
  0.571 0.031
  0.592 0.029
  0.612 0.027
  0.633 0.025
  0.653 0.023
  0.673 0.021
  0.694 0.021
  0.714 0.021
  0.735 0.021
  0.755 0.023
  0.776 0.025
  0.796 0.028
  0.816 0.032
  0.837 0.037
  0.857 0.042
  0.878 0.047
  0.898 0.051
  0.918 0.056
  0.939 0.059
  0.959 0.062
  0.980 0.064
  1.000 0.065
  /
\end{sparkline}
\\
DoRA\_Small &
0.197 &
0.000 &
0.000 &
1.000 &
\begin{sparkline}{9}
\sparkdot 0.197 0.227 red
\spark
  0.000 0.386
  0.020 0.386
  0.041 0.381
  0.061 0.372
  0.082 0.357
  0.102 0.339
  0.122 0.318
  0.143 0.294
  0.163 0.269
  0.184 0.244
  0.204 0.218
  0.224 0.194
  0.245 0.170
  0.265 0.149
  0.286 0.129
  0.306 0.112
  0.327 0.096
  0.347 0.083
  0.367 0.071
  0.388 0.061
  0.408 0.053
  0.429 0.046
  0.449 0.040
  0.469 0.035
  0.490 0.031
  0.510 0.028
  0.531 0.025
  0.551 0.023
  0.571 0.021
  0.592 0.020
  0.612 0.019
  0.633 0.019
  0.653 0.020
  0.673 0.021
  0.694 0.023
  0.714 0.026
  0.735 0.029
  0.755 0.033
  0.776 0.038
  0.796 0.043
  0.816 0.048
  0.837 0.054
  0.857 0.060
  0.878 0.065
  0.898 0.070
  0.918 0.075
  0.939 0.079
  0.959 0.082
  0.980 0.083
  1.000 0.084
  /
\end{sparkline}
\\
pash\_f3 &
0.946 &
1.000 &
1.000 &
1.000 &
\begin{sparkline}{9}
\sparkdot 0.946 0.732 red
\spark
  0.000 0.018
  0.020 0.018
  0.041 0.017
  0.061 0.016
  0.082 0.015
  0.102 0.015
  0.122 0.015
  0.143 0.016
  0.163 0.017
  0.184 0.020
  0.204 0.023
  0.224 0.026
  0.245 0.029
  0.265 0.031
  0.286 0.033
  0.306 0.033
  0.327 0.032
  0.347 0.031
  0.367 0.030
  0.388 0.028
  0.408 0.026
  0.429 0.025
  0.449 0.024
  0.469 0.023
  0.490 0.022
  0.510 0.020
  0.531 0.018
  0.551 0.016
  0.571 0.013
  0.592 0.011
  0.612 0.008
  0.633 0.006
  0.653 0.005
  0.673 0.004
  0.694 0.004
  0.714 0.006
  0.735 0.011
  0.755 0.021
  0.776 0.038
  0.796 0.065
  0.816 0.107
  0.837 0.166
  0.857 0.245
  0.878 0.344
  0.898 0.458
  0.918 0.579
  0.939 0.694
  0.959 0.791
  0.980 0.855
  1.000 0.877
  /
\end{sparkline}
\\
pash\_r2 &
0.958 &
1.000 &
1.000 &
1.000 &
\begin{sparkline}{9}
\sparkdot 0.958 0.866 red
\spark
  0.000 0.020
  0.020 0.019
  0.041 0.018
  0.061 0.016
  0.082 0.014
  0.102 0.012
  0.122 0.012
  0.143 0.012
  0.163 0.013
  0.184 0.015
  0.204 0.017
  0.224 0.019
  0.245 0.020
  0.265 0.019
  0.286 0.018
  0.306 0.016
  0.327 0.014
  0.347 0.013
  0.367 0.012
  0.388 0.012
  0.408 0.013
  0.429 0.015
  0.449 0.017
  0.469 0.019
  0.490 0.019
  0.510 0.019
  0.531 0.018
  0.551 0.016
  0.571 0.013
  0.592 0.010
  0.612 0.007
  0.633 0.005
  0.653 0.003
  0.673 0.002
  0.694 0.002
  0.714 0.003
  0.735 0.005
  0.755 0.010
  0.776 0.021
  0.796 0.042
  0.816 0.076
  0.837 0.130
  0.857 0.209
  0.878 0.316
  0.898 0.448
  0.918 0.595
  0.939 0.743
  0.959 0.870
  0.980 0.957
  1.000 0.988
  /
\end{sparkline}
\\
pinganNLP1 &
0.942 &
1.000 &
1.000 &
1.000 &
\begin{sparkline}{9}
\sparkdot 0.942 0.682 red
\spark
  0.000 0.022
  0.020 0.024
  0.041 0.026
  0.061 0.028
  0.082 0.030
  0.102 0.032
  0.122 0.034
  0.143 0.035
  0.163 0.035
  0.184 0.035
  0.204 0.033
  0.224 0.031
  0.245 0.028
  0.265 0.024
  0.286 0.020
  0.306 0.017
  0.327 0.014
  0.347 0.012
  0.367 0.012
  0.388 0.012
  0.408 0.013
  0.429 0.014
  0.449 0.015
  0.469 0.016
  0.490 0.017
  0.510 0.016
  0.531 0.016
  0.551 0.014
  0.571 0.012
  0.592 0.010
  0.612 0.008
  0.633 0.007
  0.653 0.006
  0.673 0.006
  0.694 0.007
  0.714 0.011
  0.735 0.019
  0.755 0.032
  0.776 0.053
  0.796 0.085
  0.816 0.131
  0.837 0.192
  0.857 0.270
  0.878 0.362
  0.898 0.465
  0.918 0.570
  0.939 0.668
  0.959 0.748
  0.980 0.801
  1.000 0.819
  /
\end{sparkline}
\\
pinganNLP2 &
0.943 &
1.000 &
1.000 &
1.000 &
\begin{sparkline}{9}
\sparkdot 0.943 0.693 red
\spark
  0.000 0.021
  0.020 0.022
  0.041 0.023
  0.061 0.025
  0.082 0.026
  0.102 0.027
  0.122 0.029
  0.143 0.030
  0.163 0.031
  0.184 0.032
  0.204 0.032
  0.224 0.031
  0.245 0.029
  0.265 0.027
  0.286 0.024
  0.306 0.022
  0.327 0.019
  0.347 0.017
  0.367 0.016
  0.388 0.015
  0.408 0.015
  0.429 0.016
  0.449 0.016
  0.469 0.017
  0.490 0.017
  0.510 0.017
  0.531 0.016
  0.551 0.014
  0.571 0.013
  0.592 0.010
  0.612 0.008
  0.633 0.007
  0.653 0.005
  0.673 0.005
  0.694 0.006
  0.714 0.010
  0.735 0.017
  0.755 0.029
  0.776 0.050
  0.796 0.081
  0.816 0.126
  0.837 0.187
  0.857 0.265
  0.878 0.359
  0.898 0.464
  0.918 0.572
  0.939 0.674
  0.959 0.757
  0.980 0.812
  1.000 0.832
  /
\end{sparkline}
\\
p\_bm25 &
0.827 &
0.250 &
1.000 &
1.000 &
\begin{sparkline}{9}
\sparkdot 0.827 0.213 red
\spark
  0.000 0.041
  0.020 0.046
  0.041 0.052
  0.061 0.057
  0.082 0.061
  0.102 0.065
  0.122 0.069
  0.143 0.071
  0.163 0.073
  0.184 0.075
  0.204 0.076
  0.224 0.076
  0.245 0.076
  0.265 0.076
  0.286 0.077
  0.306 0.077
  0.327 0.078
  0.347 0.080
  0.367 0.081
  0.388 0.083
  0.408 0.085
  0.429 0.087
  0.449 0.088
  0.469 0.088
  0.490 0.088
  0.510 0.086
  0.531 0.083
  0.551 0.080
  0.571 0.075
  0.592 0.071
  0.612 0.067
  0.633 0.065
  0.653 0.064
  0.673 0.065
  0.694 0.070
  0.714 0.079
  0.735 0.092
  0.755 0.110
  0.776 0.134
  0.796 0.162
  0.816 0.195
  0.837 0.231
  0.857 0.269
  0.878 0.309
  0.898 0.346
  0.918 0.381
  0.939 0.411
  0.959 0.433
  0.980 0.447
  1.000 0.452
  /
\end{sparkline}
\\
p\_d2q\_rm3\_duo &
0.949 &
1.000 &
1.000 &
1.000 &
\begin{sparkline}{9}
\sparkdot 0.949 0.775 red
\spark
  0.000 0.005
  0.020 0.007
  0.041 0.010
  0.061 0.013
  0.082 0.017
  0.102 0.021
  0.122 0.025
  0.143 0.028
  0.163 0.032
  0.184 0.034
  0.204 0.036
  0.224 0.038
  0.245 0.039
  0.265 0.039
  0.286 0.038
  0.306 0.037
  0.327 0.035
  0.347 0.033
  0.367 0.030
  0.388 0.028
  0.408 0.026
  0.429 0.025
  0.449 0.024
  0.469 0.023
  0.490 0.022
  0.510 0.021
  0.531 0.019
  0.551 0.016
  0.571 0.013
  0.592 0.010
  0.612 0.008
  0.633 0.005
  0.653 0.004
  0.673 0.003
  0.694 0.003
  0.714 0.004
  0.735 0.007
  0.755 0.014
  0.776 0.027
  0.796 0.049
  0.816 0.086
  0.837 0.142
  0.857 0.221
  0.878 0.324
  0.898 0.447
  0.918 0.583
  0.939 0.716
  0.959 0.830
  0.980 0.906
  1.000 0.934
  /
\end{sparkline}
\\
terrier{-}BM25 &
0.805 &
0.275 &
1.000 &
1.000 &
\begin{sparkline}{9}
\sparkdot 0.805 0.174 red
\spark
  0.000 0.043
  0.020 0.047
  0.041 0.051
  0.061 0.056
  0.082 0.060
  0.102 0.063
  0.122 0.066
  0.143 0.069
  0.163 0.072
  0.184 0.075
  0.204 0.077
  0.224 0.079
  0.245 0.082
  0.265 0.084
  0.286 0.087
  0.306 0.090
  0.327 0.093
  0.347 0.097
  0.367 0.100
  0.388 0.103
  0.408 0.105
  0.429 0.107
  0.449 0.108
  0.469 0.107
  0.490 0.106
  0.510 0.103
  0.531 0.099
  0.551 0.094
  0.571 0.089
  0.592 0.084
  0.612 0.079
  0.633 0.076
  0.653 0.074
  0.673 0.075
  0.694 0.079
  0.714 0.087
  0.735 0.099
  0.755 0.115
  0.776 0.136
  0.796 0.162
  0.816 0.191
  0.837 0.223
  0.857 0.257
  0.878 0.292
  0.898 0.325
  0.918 0.355
  0.939 0.381
  0.959 0.400
  0.980 0.412
  1.000 0.416
  /
\end{sparkline}
\\
terrier{-}DPH &
0.791 &
0.333 &
1.000 &
1.000 &
\begin{sparkline}{9}
\sparkdot 0.791 0.152 red
\spark
  0.000 0.035
  0.020 0.039
  0.041 0.044
  0.061 0.049
  0.082 0.054
  0.102 0.059
  0.122 0.066
  0.143 0.072
  0.163 0.079
  0.184 0.086
  0.204 0.093
  0.224 0.100
  0.245 0.106
  0.265 0.112
  0.286 0.117
  0.306 0.122
  0.327 0.125
  0.347 0.127
  0.367 0.128
  0.388 0.128
  0.408 0.126
  0.429 0.124
  0.449 0.120
  0.469 0.115
  0.490 0.109
  0.510 0.103
  0.531 0.096
  0.551 0.089
  0.571 0.082
  0.592 0.076
  0.612 0.071
  0.633 0.068
  0.653 0.067
  0.673 0.068
  0.694 0.073
  0.714 0.082
  0.735 0.095
  0.755 0.111
  0.776 0.133
  0.796 0.158
  0.816 0.186
  0.837 0.217
  0.857 0.250
  0.878 0.283
  0.898 0.314
  0.918 0.343
  0.939 0.367
  0.959 0.385
  0.980 0.396
  1.000 0.400
  /
\end{sparkline}
\\
\bottomrule
\end{tabular}


==> robust-example.tex <==
\begin{tabular}{lccccc}
System
& Mean
& 10\%ile
& Median
& 90\%ile
& Dist. (KDE) \\
\toprule
humR04d4 &
0.418 &
0.063 &
0.431 &
0.791 &
\begin{sparkline}{9}
\sparkdot 0.418 0.944 red
\spark
  0.000 0.506
  0.020 0.585
  0.041 0.656
  0.061 0.716
  0.082 0.764
  0.102 0.800
  0.122 0.826
  0.143 0.842
  0.163 0.851
  0.184 0.853
  0.204 0.849
  0.224 0.842
  0.245 0.832
  0.265 0.823
  0.286 0.817
  0.306 0.817
  0.327 0.826
  0.347 0.843
  0.367 0.867
  0.388 0.897
  0.408 0.929
  0.429 0.959
  0.449 0.982
  0.469 0.997
  0.490 0.999
  0.510 0.990
  0.531 0.968
  0.551 0.935
  0.571 0.895
  0.592 0.850
  0.612 0.803
  0.633 0.755
  0.653 0.709
  0.673 0.665
  0.694 0.625
  0.714 0.589
  0.735 0.557
  0.755 0.528
  0.776 0.502
  0.796 0.477
  0.816 0.452
  0.837 0.425
  0.857 0.396
  0.878 0.365
  0.898 0.330
  0.918 0.293
  0.939 0.254
  0.959 0.215
  0.980 0.177
  1.000 0.141
  /
\end{sparkline}
\\
humR04d5 &
0.401 &
0.081 &
0.393 &
0.751 &
\begin{sparkline}{9}
\sparkdot 0.401 0.995 red
\spark
  0.000 0.458
  0.020 0.552
  0.041 0.644
  0.061 0.728
  0.082 0.800
  0.102 0.859
  0.122 0.904
  0.143 0.933
  0.163 0.950
  0.184 0.955
  0.204 0.952
  0.224 0.943
  0.245 0.933
  0.265 0.925
  0.286 0.923
  0.306 0.928
  0.327 0.940
  0.347 0.956
  0.367 0.974
  0.388 0.988
  0.408 0.998
  0.429 1.000
  0.449 0.993
  0.469 0.979
  0.490 0.957
  0.510 0.929
  0.531 0.896
  0.551 0.859
  0.571 0.820
  0.592 0.780
  0.612 0.740
  0.633 0.701
  0.653 0.664
  0.673 0.629
  0.694 0.595
  0.714 0.563
  0.735 0.531
  0.755 0.499
  0.776 0.467
  0.796 0.435
  0.816 0.401
  0.837 0.367
  0.857 0.331
  0.878 0.295
  0.898 0.258
  0.918 0.220
  0.939 0.184
  0.959 0.149
  0.980 0.118
  1.000 0.090
  /
\end{sparkline}
\\
humR04t1 &
0.412 &
0.100 &
0.404 &
0.752 &
\begin{sparkline}{9}
\sparkdot 0.412 0.995 red
\spark
  0.000 0.317
  0.020 0.389
  0.041 0.460
  0.061 0.527
  0.082 0.587
  0.102 0.639
  0.122 0.682
  0.143 0.718
  0.163 0.747
  0.184 0.771
  0.204 0.791
  0.224 0.809
  0.245 0.824
  0.265 0.840
  0.286 0.858
  0.306 0.878
  0.327 0.902
  0.347 0.928
  0.367 0.954
  0.388 0.976
  0.408 0.993
  0.429 1.000
  0.449 0.996
  0.469 0.979
  0.490 0.950
  0.510 0.911
  0.531 0.862
  0.551 0.806
  0.571 0.747
  0.592 0.687
  0.612 0.630
  0.633 0.579
  0.653 0.535
  0.673 0.498
  0.694 0.468
  0.714 0.442
  0.735 0.419
  0.755 0.394
  0.776 0.368
  0.796 0.341
  0.816 0.313
  0.837 0.286
  0.857 0.261
  0.878 0.237
  0.898 0.215
  0.918 0.192
  0.939 0.168
  0.959 0.143
  0.980 0.117
  1.000 0.092
  /
\end{sparkline}
\\
icl04pos2t &
0.292 &
0.052 &
0.247 &
0.609 &
\begin{sparkline}{9}
\sparkdot 0.292 0.844 red
\spark
  0.000 0.554
  0.020 0.669
  0.041 0.775
  0.061 0.863
  0.082 0.929
  0.102 0.973
  0.122 0.995
  0.143 1.000
  0.163 0.991
  0.184 0.975
  0.204 0.953
  0.224 0.929
  0.245 0.904
  0.265 0.879
  0.286 0.852
  0.306 0.823
  0.327 0.790
  0.347 0.754
  0.367 0.715
  0.388 0.674
  0.408 0.634
  0.429 0.594
  0.449 0.555
  0.469 0.517
  0.490 0.479
  0.510 0.442
  0.531 0.406
  0.551 0.372
  0.571 0.339
  0.592 0.307
  0.612 0.275
  0.633 0.244
  0.653 0.214
  0.673 0.187
  0.694 0.166
  0.714 0.151
  0.735 0.143
  0.755 0.140
  0.776 0.141
  0.796 0.141
  0.816 0.140
  0.837 0.134
  0.857 0.124
  0.878 0.111
  0.898 0.095
  0.918 0.079
  0.939 0.063
  0.959 0.048
  0.980 0.035
  1.000 0.025
  /
\end{sparkline}
\\
JuruDesTrSl &
0.424 &
0.091 &
0.410 &
0.771 &
\begin{sparkline}{9}
\sparkdot 0.424 0.948 red
\spark
  0.000 0.437
  0.020 0.516
  0.041 0.590
  0.061 0.657
  0.082 0.714
  0.102 0.762
  0.122 0.802
  0.143 0.836
  0.163 0.867
  0.184 0.895
  0.204 0.921
  0.224 0.945
  0.245 0.966
  0.265 0.982
  0.286 0.994
  0.306 0.999
  0.327 0.999
  0.347 0.994
  0.367 0.984
  0.388 0.971
  0.408 0.957
  0.429 0.946
  0.449 0.940
  0.469 0.941
  0.490 0.947
  0.510 0.956
  0.531 0.964
  0.551 0.966
  0.571 0.958
  0.592 0.937
  0.612 0.904
  0.633 0.860
  0.653 0.810
  0.673 0.756
  0.694 0.701
  0.714 0.649
  0.735 0.599
  0.755 0.552
  0.776 0.508
  0.796 0.465
  0.816 0.426
  0.837 0.389
  0.857 0.354
  0.878 0.323
  0.898 0.294
  0.918 0.266
  0.939 0.238
  0.959 0.210
  0.980 0.181
  1.000 0.151
  /
\end{sparkline}
\\
mpi04r02 &
0.187 &
0.000 &
0.137 &
0.445 &
\begin{sparkline}{9}
\sparkdot 0.187 0.684 red
\spark
  0.000 0.823
  0.020 0.933
  0.041 0.990
  0.061 0.998
  0.082 0.969
  0.102 0.920
  0.122 0.864
  0.143 0.808
  0.163 0.751
  0.184 0.692
  0.204 0.631
  0.224 0.569
  0.245 0.512
  0.265 0.464
  0.286 0.427
  0.306 0.401
  0.327 0.381
  0.347 0.363
  0.367 0.343
  0.388 0.320
  0.408 0.297
  0.429 0.272
  0.449 0.248
  0.469 0.224
  0.490 0.200
  0.510 0.178
  0.531 0.157
  0.551 0.138
  0.571 0.120
  0.592 0.105
  0.612 0.091
  0.633 0.078
  0.653 0.066
  0.673 0.055
  0.694 0.047
  0.714 0.040
  0.735 0.035
  0.755 0.032
  0.776 0.030
  0.796 0.029
  0.816 0.027
  0.837 0.025
  0.857 0.021
  0.878 0.017
  0.898 0.012
  0.918 0.008
  0.939 0.005
  0.959 0.003
  0.980 0.001
  1.000 0.001
  /
\end{sparkline}
\\
mpi04r05 &
0.311 &
0.015 &
0.281 &
0.638 &
\begin{sparkline}{9}
\sparkdot 0.311 0.969 red
\spark
  0.000 0.647
  0.020 0.730
  0.041 0.796
  0.061 0.847
  0.082 0.884
  0.102 0.911
  0.122 0.932
  0.143 0.948
  0.163 0.963
  0.184 0.975
  0.204 0.986
  0.224 0.994
  0.245 0.999
  0.265 0.999
  0.286 0.991
  0.306 0.974
  0.327 0.948
  0.347 0.913
  0.367 0.870
  0.388 0.821
  0.408 0.769
  0.429 0.716
  0.449 0.666
  0.469 0.619
  0.490 0.579
  0.510 0.545
  0.531 0.519
  0.551 0.499
  0.571 0.483
  0.592 0.468
  0.612 0.451
  0.633 0.430
  0.653 0.403
  0.673 0.370
  0.694 0.333
  0.714 0.294
  0.735 0.255
  0.755 0.220
  0.776 0.189
  0.796 0.164
  0.816 0.144
  0.837 0.128
  0.857 0.115
  0.878 0.103
  0.898 0.092
  0.918 0.079
  0.939 0.066
  0.959 0.053
  0.980 0.041
  1.000 0.030
  /
\end{sparkline}
\\
NLPR04clus10 &
0.461 &
0.166 &
0.454 &
0.774 &
\begin{sparkline}{9}
\sparkdot 0.461 1.000 red
\spark
  0.000 0.147
  0.020 0.197
  0.041 0.254
  0.061 0.315
  0.082 0.378
  0.102 0.438
  0.122 0.493
  0.143 0.542
  0.163 0.584
  0.184 0.622
  0.204 0.658
  0.224 0.694
  0.245 0.731
  0.265 0.769
  0.286 0.807
  0.306 0.844
  0.327 0.879
  0.347 0.910
  0.367 0.937
  0.388 0.959
  0.408 0.977
  0.429 0.990
  0.449 0.998
  0.469 1.000
  0.490 0.992
  0.510 0.975
  0.531 0.946
  0.551 0.908
  0.571 0.860
  0.592 0.805
  0.612 0.747
  0.633 0.690
  0.653 0.638
  0.673 0.592
  0.694 0.554
  0.714 0.522
  0.735 0.494
  0.755 0.468
  0.776 0.439
  0.796 0.409
  0.816 0.377
  0.837 0.344
  0.857 0.313
  0.878 0.283
  0.898 0.256
  0.918 0.230
  0.939 0.203
  0.959 0.175
  0.980 0.146
  1.000 0.116
  /
\end{sparkline}
\\
NLPR04COMB &
0.445 &
0.109 &
0.451 &
0.777 &
\begin{sparkline}{9}
\sparkdot 0.445 0.969 red
\spark
  0.000 0.278
  0.020 0.350
  0.041 0.423
  0.061 0.493
  0.082 0.554
  0.102 0.604
  0.122 0.642
  0.143 0.668
  0.163 0.685
  0.184 0.696
  0.204 0.707
  0.224 0.720
  0.245 0.736
  0.265 0.756
  0.286 0.779
  0.306 0.804
  0.327 0.828
  0.347 0.851
  0.367 0.875
  0.388 0.899
  0.408 0.924
  0.429 0.950
  0.449 0.974
  0.469 0.992
  0.490 1.000
  0.510 0.994
  0.531 0.973
  0.551 0.936
  0.571 0.886
  0.592 0.827
  0.612 0.764
  0.633 0.702
  0.653 0.643
  0.673 0.590
  0.694 0.545
  0.714 0.505
  0.735 0.471
  0.755 0.441
  0.776 0.413
  0.796 0.388
  0.816 0.364
  0.837 0.342
  0.857 0.322
  0.878 0.304
  0.898 0.285
  0.918 0.265
  0.939 0.242
  0.959 0.216
  0.980 0.187
  1.000 0.155
  /
\end{sparkline}
\\
NLPR04LcA &
0.445 &
0.109 &
0.454 &
0.777 &
\begin{sparkline}{9}
\sparkdot 0.445 0.973 red
\spark
  0.000 0.273
  0.020 0.344
  0.041 0.416
  0.061 0.485
  0.082 0.547
  0.102 0.597
  0.122 0.635
  0.143 0.661
  0.163 0.678
  0.184 0.690
  0.204 0.701
  0.224 0.713
  0.245 0.728
  0.265 0.748
  0.286 0.772
  0.306 0.798
  0.327 0.824
  0.347 0.850
  0.367 0.876
  0.388 0.902
  0.408 0.929
  0.429 0.954
  0.449 0.977
  0.469 0.994
  0.490 1.000
  0.510 0.992
  0.531 0.968
  0.551 0.929
  0.571 0.876
  0.592 0.814
  0.612 0.748
  0.633 0.684
  0.653 0.625
  0.673 0.574
  0.694 0.531
  0.714 0.496
  0.735 0.466
  0.755 0.440
  0.776 0.416
  0.796 0.392
  0.816 0.369
  0.837 0.347
  0.857 0.325
  0.878 0.305
  0.898 0.284
  0.918 0.262
  0.939 0.238
  0.959 0.212
  0.980 0.182
  1.000 0.151
  /
\end{sparkline}
\\
pircRB04t3 &
0.502 &
0.187 &
0.501 &
0.823 &
\begin{sparkline}{9}
\sparkdot 0.502 0.998 red
\spark
  0.000 0.167
  0.020 0.215
  0.041 0.266
  0.061 0.317
  0.082 0.365
  0.102 0.411
  0.122 0.454
  0.143 0.495
  0.163 0.536
  0.184 0.580
  0.204 0.626
  0.224 0.674
  0.245 0.721
  0.265 0.765
  0.286 0.804
  0.306 0.838
  0.327 0.867
  0.347 0.892
  0.367 0.914
  0.388 0.936
  0.408 0.956
  0.429 0.974
  0.449 0.988
  0.469 0.997
  0.490 1.000
  0.510 0.995
  0.531 0.982
  0.551 0.963
  0.571 0.937
  0.592 0.908
  0.612 0.878
  0.633 0.848
  0.653 0.822
  0.673 0.800
  0.694 0.782
  0.714 0.767
  0.735 0.753
  0.755 0.735
  0.776 0.712
  0.796 0.681
  0.816 0.641
  0.837 0.593
  0.857 0.541
  0.878 0.485
  0.898 0.429
  0.918 0.375
  0.939 0.322
  0.959 0.271
  0.980 0.222
  1.000 0.177
  /
\end{sparkline}
\\
SABIR04BA &
0.464 &
0.143 &
0.476 &
0.766 &
\begin{sparkline}{9}
\sparkdot 0.464 0.992 red
\spark
  0.000 0.247
  0.020 0.291
  0.041 0.333
  0.061 0.373
  0.082 0.411
  0.102 0.446
  0.122 0.479
  0.143 0.510
  0.163 0.539
  0.184 0.565
  0.204 0.588
  0.224 0.611
  0.245 0.634
  0.265 0.659
  0.286 0.688
  0.306 0.721
  0.327 0.758
  0.347 0.799
  0.367 0.842
  0.388 0.884
  0.408 0.923
  0.429 0.956
  0.449 0.981
  0.469 0.996
  0.490 1.000
  0.510 0.994
  0.531 0.978
  0.551 0.955
  0.571 0.926
  0.592 0.893
  0.612 0.858
  0.633 0.820
  0.653 0.779
  0.673 0.735
  0.694 0.689
  0.714 0.639
  0.735 0.587
  0.755 0.534
  0.776 0.482
  0.796 0.432
  0.816 0.386
  0.837 0.345
  0.857 0.309
  0.878 0.277
  0.898 0.247
  0.918 0.219
  0.939 0.192
  0.959 0.165
  0.980 0.139
  1.000 0.113
  /
\end{sparkline}
\\
uogRobLT &
0.464 &
0.079 &
0.473 &
0.807 &
\begin{sparkline}{9}
\sparkdot 0.464 0.986 red
\spark
  0.000 0.456
  0.020 0.513
  0.041 0.560
  0.061 0.597
  0.082 0.625
  0.102 0.646
  0.122 0.661
  0.143 0.675
  0.163 0.689
  0.184 0.704
  0.204 0.722
  0.224 0.740
  0.245 0.760
  0.265 0.781
  0.286 0.803
  0.306 0.824
  0.327 0.847
  0.347 0.870
  0.367 0.893
  0.388 0.916
  0.408 0.938
  0.429 0.959
  0.449 0.976
  0.469 0.988
  0.490 0.997
  0.510 1.000
  0.531 0.999
  0.551 0.994
  0.571 0.986
  0.592 0.976
  0.612 0.963
  0.633 0.949
  0.653 0.933
  0.673 0.914
  0.694 0.894
  0.714 0.870
  0.735 0.842
  0.755 0.808
  0.776 0.768
  0.796 0.722
  0.816 0.669
  0.837 0.612
  0.857 0.552
  0.878 0.491
  0.898 0.431
  0.918 0.374
  0.939 0.320
  0.959 0.270
  0.980 0.223
  1.000 0.180
  /
\end{sparkline}
\\
uogRobLWR10 &
0.472 &
0.067 &
0.490 &
0.812 &
\begin{sparkline}{9}
\sparkdot 0.472 0.988 red
\spark
  0.000 0.466
  0.020 0.525
  0.041 0.575
  0.061 0.614
  0.082 0.643
  0.102 0.664
  0.122 0.678
  0.143 0.688
  0.163 0.697
  0.184 0.705
  0.204 0.713
  0.224 0.724
  0.245 0.737
  0.265 0.754
  0.286 0.773
  0.306 0.796
  0.327 0.822
  0.347 0.850
  0.367 0.879
  0.388 0.907
  0.408 0.933
  0.429 0.955
  0.449 0.973
  0.469 0.986
  0.490 0.995
  0.510 0.999
  0.531 1.000
  0.551 0.998
  0.571 0.995
  0.592 0.990
  0.612 0.985
  0.633 0.979
  0.653 0.973
  0.673 0.966
  0.694 0.957
  0.714 0.945
  0.735 0.927
  0.755 0.902
  0.776 0.867
  0.796 0.821
  0.816 0.765
  0.837 0.701
  0.857 0.630
  0.878 0.556
  0.898 0.482
  0.918 0.411
  0.939 0.345
  0.959 0.285
  0.980 0.231
  1.000 0.183
  /
\end{sparkline}
\\
vtumlong432 &
0.489 &
0.123 &
0.496 &
0.833 &
\begin{sparkline}{9}
\sparkdot 0.489 0.973 red
\spark
  0.000 0.283
  0.020 0.335
  0.041 0.383
  0.061 0.425
  0.082 0.459
  0.102 0.485
  0.122 0.506
  0.143 0.522
  0.163 0.535
  0.184 0.547
  0.204 0.559
  0.224 0.570
  0.245 0.584
  0.265 0.601
  0.286 0.622
  0.306 0.649
  0.327 0.683
  0.347 0.722
  0.367 0.765
  0.388 0.810
  0.408 0.854
  0.429 0.893
  0.449 0.926
  0.469 0.953
  0.490 0.973
  0.510 0.988
  0.531 0.998
  0.551 1.000
  0.571 0.994
  0.592 0.977
  0.612 0.948
  0.633 0.909
  0.653 0.860
  0.673 0.806
  0.694 0.751
  0.714 0.700
  0.735 0.654
  0.755 0.615
  0.776 0.582
  0.796 0.552
  0.816 0.523
  0.837 0.493
  0.857 0.461
  0.878 0.426
  0.898 0.388
  0.918 0.349
  0.939 0.308
  0.959 0.267
  0.980 0.226
  1.000 0.185
  /
\end{sparkline}
\\
vtumtitle &
0.430 &
0.030 &
0.431 &
0.796 &
\begin{sparkline}{9}
\sparkdot 0.430 0.982 red
\spark
  0.000 0.638
  0.020 0.700
  0.041 0.748
  0.061 0.782
  0.082 0.804
  0.102 0.819
  0.122 0.830
  0.143 0.840
  0.163 0.851
  0.184 0.862
  0.204 0.874
  0.224 0.884
  0.245 0.893
  0.265 0.901
  0.286 0.909
  0.306 0.917
  0.327 0.927
  0.347 0.939
  0.367 0.951
  0.388 0.963
  0.408 0.974
  0.429 0.981
  0.449 0.987
  0.469 0.990
  0.490 0.991
  0.510 0.992
  0.531 0.994
  0.551 0.996
  0.571 0.999
  0.592 1.000
  0.612 0.998
  0.633 0.991
  0.653 0.977
  0.673 0.954
  0.694 0.922
  0.714 0.881
  0.735 0.833
  0.755 0.779
  0.776 0.721
  0.796 0.662
  0.816 0.603
  0.837 0.545
  0.857 0.490
  0.878 0.438
  0.898 0.388
  0.918 0.341
  0.939 0.297
  0.959 0.254
  0.980 0.214
  1.000 0.175
  /
\end{sparkline}
\\
\bottomrule
\end{tabular}

